A 5deg x 5deg deep HI survey of the M81 group

A 25 $\rm deg^2$ region, including the M81 complex (M81, M82, NGC 3077), NGC 2976 and IC2574, was mapped during ~3000 hours with the DRAO synthesis telescope. With a physical resolution of ~1 kpc, these observations allow us to probe a large region down to column density levels of ~$\rm 1\times10^{18}\, cm^{-2}$ over 16 $\rm km\, s^{-1}$, mapping the extent of the HI arm connecting the system and NGC 2976, and resolving the HI clouds adjacent to the arm. The observations also reveal a few clouds located between the system and IC 2574, probably tidally stripped from a past interaction between the two systems. Given the regular velocity distribution in the HI envelope of the system, we attempt and derive an idealised large-scale rotation curve of the system. We observe a flat trend for the rotation velocity of the overall system from 20 kpc out to 80 kpc, well beyond the outskirts of the M81 disk, although with asymmetries like a wiggle at the vicinity of M82. This supports the assumption that intergalactic gas and galaxies in the system participate to a large-scale ordered rotation motion which is dominated by M81. Also, our HI analysis of the group further supports the hypothesis that the galaxies forming the system moved closer from afar, in agreement with numerical simulations.

==> view.tex <==
VIEW=front
COO=-7480.873046875 1540.5379638671875 7583.59814453125
C2C=0.01647897996008396 0.0042088269256055355 -0.9998553395271301
ROO=172940.65386715755
ROLL=-103.0665095565494
LIGHTS=Cube
END
VIEW=right
COO=-4523.0673828125 3750.296142578125 6615.30908203125
C2C=0.9974812865257263 -0.06800006330013275 -0.020179886370897293
ROO=174133.35064828908
ROLL=-89.44795929500106
LIGHTS=Cube
END
VIEW=left
COO=-12007.8994140625 -943.5294189453125 5836.46826171875
C2C=-0.9978785514831543 0.0637609139084816 -0.01315404288470745
ROO=118935.33893675168
ROLL=89.02146179265795
LIGHTS=Cube
END
VIEW=back
COO=-9956.5244140625 966.1571655273438 8360.8974609375
C2C=0.018802549690008163 -0.057195547968149185 0.998185932636261
ROO=162667.95785279904
ROLL=-162.74981584495552
LIGHTS=Cube
END
VIEW=top
COO=-6271.14404296875 3742.04736328125 6677.79638671875
C2C=0.07051078975200653 -0.9971247911453247 -0.02775450423359871
ROO=149527.91589532705
ROLL=-0.014670559316206422
LIGHTS=Cube
END
VIEW=bottom 
COO=-6295.3232421875 3538.95947265625 6225.33203125
C2C=-0.0376497246325016 0.9978257417678833 -0.05409638583660126
ROO=154648.73974268266
ROLL=-178.87064689007306
LIGHTS=Cube
END

